Space Debris Reliable Capturing by a Dual-Arm Orbital Robot: Detumbling and Caging

A chaser satellite equipped with robotic arms can capture space debris and manipulate it for use in more advanced missions such as refueling and deorbiting. To facilitate capturing, a caging-based strategy has been proposed to simplify the control system. Caging involves geometrically constraining the motion of the target debris, and is achieved via position control. However, if the target is spinning at a high speed, direct caging may result in unsuccessful constraints or hardware destruction; therefore, the target should be de-tumbled before capture. To address this problem, this study proposes a repeated contact-based method that uses impedance control to mitigate the momentum of the target. In this study, we analyzed the proposed detumbling technique from the perspective of impedance parameters. We investigated their effects through a parametric analysis and demonstrated the successful detumbling and caging sequence of a microsatellite as representative of space debris. The contact forces decreased during the detumbling sequence compared with direct caging. Further, the proposed detumbling and caging sequence was validated through simulations and experiments using a dual-arm air-floating robot in two-dimensional microgravity emulating testbed.

==> macrosForEThesis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   macrosForEThesis.tex
%%   -------------------
%%
%%   Title: LaTeX macro file for the English Thesis
%%   
%%   
%%   Belief:
%%   1."Fig. 1: ~~~", "Table 1: ~~~" are for the figure and table citation.
%%   2. add the config to read the source code file (hello.c) and visualize it. 
%%
%%   Change Log:
%%   2020.11.26 Initial creation by Kentaro UNO
%%
%%   Contact:
%%   Please contact the author Kentaro UNO (unoken.astro@gmail.com) if
%%   you have a problem
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% useful command
\newcommand{\n}{\nonumber \\}
\newcommand{\p}{\partial}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\II}{I\negthinspace I}
\newcommand{\III}{I\negthinspace I\negthinspace I}
\newcommand{\mbm}[1]{\mbox{\protect \boldmath $#1$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  config for citation of figures, tables, and equations
%%%  to use English for all. 
%%%  2020.01.29 modified by Kentaro UNO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% figure and table
\captionsetup{compatibility=false}
%
\renewcommand{\figurename}{Fig.~\hspace{-.2em}}   
\renewcommand{\tablename}{Table~\hspace{-.2em}}

\captionsetup[figure]{format=plain,labelformat=simple,labelsep=colon,font=small}
\captionsetup[table]{format=plain,labelformat=simple,labelsep=colon,font=small}

\newcommand{\bhline}[1]{\noalign{\hrule height #1}} % bhlineコマンドの設定

%%% citation command for figures, tables, and equations
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\subfig}[2]{Fig.~\ref{#1}\subref{#2}}
\newcommand{\fign}[1]{\ref{#1}}
\newcommand{\tb}[1]{Table~\ref{#1}}
\newcommand{\tabn}[1]{\ref{#1}}
\newcommand{\eq}[1]{Eq.~(\ref{#1})}
\newcommand{\eqn}[1]{(\ref{#1})}

%%% citation command for chapters, sections, and appendixes
\newcommand{\chap}[1]{Chap.~\ref{#1}}
\newcommand{\sect}[1]{Sect.~\ref{#1}}
\newcommand{\subsect}[1]{Sect.~\ref{#1}}
\newcommand{\app}[1]{Appnd. ~\ref{#1}}

%%% visualize a figure and table in a row
\makeatletter
\newcommand{\figcaption}[1]{\def\@captype{figure}\caption{#1}}
\newcommand{\tblcaption}[1]{\def\@captype{table}\caption{#1}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  ソースコードの引用スタイルの設定
%%%  2020.01.24 added by Kentaro UNO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings} %日本語のコメントアウトをする場合はjlistingが必要
%ここからソースコードの表示に関する設定
\definecolor{gray}{rgb}{0.9,0.9,0.9}
\lstset{
  backgroundcolor=\color{gray}, % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle={\small\ttfamily}, % the style of the fonts that are used for the code
  identifierstyle={\small}, % main()の''main''等のスタイル
  commentstyle={\small\itshape}, %//comment 等のスタイル
  keywordstyle={\small}, % int mainの''int''等のスタイル
  ndkeywordstyle={\small},
  stringstyle={\small\ttfamily},  % string literal style -> % printf(''Hello'')の''''で囲まれた部分のスタイル
  %frame={tb},
  breaklines=true, % sets automatic line breaking
  columns=[l]{fullflexible},
  numbers=left, % where to put the line-numbers; possible values are (none, left, right)
  numberstyle={\scriptsize}, % the style that is used for the line-numbers
  stepnumber=1, % the step between two line-numbers. If it's 1, each line will be numbered
  numbersep=1zw, % 行数字とコードの間のマージン
  xrightmargin=0zw, % 表示個所の右側マージン
  xleftmargin=2zw,  % 表示個所の左側マージン
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  lineskip=-0.5ex % codeの行間の設定
}

\def\epsgaiji#1{\leavevmode\kern-0.025zw\raise-.37zh\hbox{%
  \epsfile{file=#1,width=1.05zw}}\kern-0.025zw}
%\newcommand{\dfrac}[2]{\frac{\displaystyle{#1}}{\displaystyle{#2}}}
\newcommand{\MARU}[1]{{\ooalign{\hfil#1\/\hfil\crcr\raise.167ex\hbox{\mathhexbox20D}}}}

%%%
